VeMo: Enabling Transparent Vehicular Mobility Modeling at Individual Levels with Full Penetration

Understanding and predicting real-time vehicle mobility patterns on highways are essential to address traffic congestion and respond to the emergency. However, almost all existing works (e.g., based on cellphones, onboard devices, or traffic cameras) suffer from high costs, low penetration rates, or only aggregate results. To address these drawbacks, we utilize Electric Toll Collection systems (ETC) as a large-scale sensor network and design a system called VeMo to transparently model and predict vehicle mobility at the individual level with a full penetration rate. Our novelty is how we address uncertainty issues (i.e., unknown routes and speeds) due to sparse implicit ETC data based on a key data-driven insight, i.e., individual driving behaviors are strongly correlated with crowds of drivers under certain spatiotemporal contexts and can be predicted by combining both personal habits and context information. More importantly, we evaluate VeMo with (i) a large-scale ETC system with tracking devices at 773 highway entrances and exits capturing more than 2 million vehicles every day; (ii) a fleet consisting of 114 thousand vehicles with GPS data as ground truth. We compared VeMo with state-of-the-art benchmark mobility models, and the experimental results show that VeMo outperforms them by average 10% in terms of accuracy.

==> 5Model_bak.tex <==

\begin{table*}[t]
\centering
\caption{Mobility Modeling Features}
\label{tb:features}
\begin{tabular}{|l|l|l|l|}
\hline
 & \begin{tabular}[c]{@{}l@{}}Individual Features\end{tabular}                           
 & \begin{tabular}[c]{@{}l@{}}Crowd Features\end{tabular} 
 & \begin{tabular}[c]{@{}l@{}}Context Features\end{tabular}        
 \\ \hline
\begin{tabular}[c]{@{}l@{}}Destination Predictor\\(Section~\ref{sec:destination_prediction})\end{tabular} & \begin{tabular}[c]{@{}l@{}}
Historical Destinations,\\ Time of Day, \\ Vehicle Type\end{tabular}   
& Crowd Destination Distributions                 
&\begin{tabular}[c]{@{}l@{}} Day of Week\\ Weekday/weekend\end{tabular} 
\\ \hline
\begin{tabular}[c]{@{}l@{}}Route Predictor\\(Section~\ref{sec:route_prediction})\end{tabular}             & \begin{tabular}[c]{@{}l@{}}Historical Routes,\\ Driving Experience,\\ Time of Day \end{tabular} & Crowd Route Distributions                                
&\begin{tabular}[c]{@{}l@{}} Day of Week\\ Traffic Speed  \end{tabular} 
\\ \hline
\begin{tabular}[c]{@{}l@{}}Speed Predictor\\(Section~\ref{sec:speed_prediction})\end{tabular}             & \begin{tabular}[c]{@{}l@{}}Historical Driving Speed,\\ Time of Day,\\ Vehicle Type\end{tabular}  
& Crowd Speed Distributions                                
& \begin{tabular}[c]{@{}l@{}}Weekday/weekend,\\ Weather\end{tabular} 
\\ \hline
\end{tabular}
\end{table*}

\section{VeMo Design}
\label{sec:model}

In this section, we first depict the overview framework of VeMo, which is then followed by feature extraction of three major components including 
(i) destination prediction, 
(ii) route inference, and
(iii) speed estimation. 
These features are fed into a learner to learn predictors for different tasks. Finally, we put them all together and provide feedback-based mechanisms to make VeMo be updated by itself.

\begin{figure}[htbp] \centering
    \begin{minipage}{0.46\textwidth} \centering
        \vspace*{-5pt}
        \includegraphics[width=\textwidth, keepaspectratio=true]{fig/model.pdf}
        \vspace*{-15pt}
    \end{minipage}
    \caption{Framework}
    \label{fig:model}
    \vspace*{-15pt}
\end{figure}

\subsection{Framework}

Figure~\ref{fig:model} shows the framework of our system, which consists of two parts: offline learning and online prediction.
\noindent In the offline learning, all the data come from three data sources including the road map, historical ETC transactions and context data.
In the feature extraction, we divide all the features into three categories, which are individual features, crowd features and context features. 
The feature summary is presented in Table~\ref{tb:features}.
By fitting these features into the learner, we train three predictors for destinations, routes and speeds. 
%It is worth mentioning that the fitted features may be different for different tasks.
In the online prediction, after the vehicles enter the system, the previously-learned predictors collaboratively predicate the vehicles' real-time locations. After the vehicles pass through the exits, the actual destination and travel duration are passed back to the predictors as feedback for online updating. The feedback mechanisms provide the ability to the system for self-calibration and revision.
In the next three subsections, we introduce three predictors for destinations, routes, and speeds from a feature perspective respectively, and then unify them together with a prediction model based on Mondrian Forest.  

% In the following sections, we will first introduce the feature extraction for three different tasks and then present the leaner used to learn three predictors. Finally, three predictors are put together to predict the real-time location. 

% The vehicle's real-time location is determined by two major components: macro factors (i.e., destination, path, total travel time) and micro factors (i.e., real-time driving speed, driving time). Macro factors control the coarse-grain locations of vehicles. For example, given the destinations and the paths, the real-time locations of vehicles cannot appear in other paths or toward other destinations. Given the total travel time, the vehicles cannot be in the middle of the path while driving time is longer than the total travel time. Micro factors control the fine-grain locations of the vehicles. For example, given the real-time driving speed and the driving time, it is easy to infer the vehicle's location in the path. Both components work collaboratively to infer the vehicle's real-time location. Figure~\ref{} gives the diagram of the workflow.



\subsection{Destination Predictor}
\label{sec:destination_prediction}
% \label{sec:dest_features}

% Almost all these works study spatial and temporal correlations to infer people's final destinations in different granularity (i.e., road level, region level, POI level). 
% Similarly, we first study vehicles' spatial and temporal correlations using historical data. 
% Figure~\ref{fig:od_boxplot} shows vehicles' possible destinations given one specific entrance at specific time in one-month transactions. 
% For example, the fifth box in the Figure~\ref{fig:od_wkday} means, there are only 3 possible destinations for $75\%$ of the vehicles between 10 am and 12 pm.
% Unlike a large number of possible destinations in the cities shown in ~\cite{xu2016destpre}, it shows vehicles have relatively stable mobility patterns on highways. 
% This insight shows the potential to predict vehicles' destinations given their historical mobility patterns.

% \begin{figure}[htbp] \centering
%     \begin{minipage}{0.46\textwidth} \centering
%         \vspace*{-10pt}
% %         \hspace*{-30pt}
%         \includegraphics[width=\textwidth, keepaspectratio=true]{fig/od_boxplot_wkday.pdf}
%         \vspace*{-15pt}
%         % \hspace*{5pt}
%     \end{minipage}
%     \caption{Number of possible destinations}
%     \label{fig:od_boxplot}
%     \vspace*{-5pt}
% \end{figure}

Destination prediction has been intensively studied in the past few years~\cite{gonzalez2008understanding,zhang2014exploring}. The existing approaches for the vehicle destination prediction mainly reply on transition probabilities between different locations through learning historical trajectories using various Markov chain based models~\cite{li2015inferring, do2012contextual}. One of the key prerequisites is that there should be enough historical data of individuals to learn the transition probabilities. However, in our context, most vehicles only have limited historical data (as we discussed in Section~\ref{sec:moti}), which makes it hard to directly apply the Markov chain based models. To address this issue, we explore more individual features, crowd features and context features as follows.  

    \textbf{Individual Features:} Since individual destinations essentially are based on individual person's habits, we utilize a set of individual features.
    \begin{itemize}
        \item \textbf{Historical Destinations:} 
        As shown in Figure~\ref{fig:dest_entropy}, 
        the mobility patterns of most individuals in terms of destinations are relatively stable. Therefore, historical destinations may largely represent their future destinations.
        \item \textbf{Time Factor:}
        Considering the commute pattern in Figure~\ref{fig:dest_entropy} when the entropy equals to 1, 
        by introducing the entering time factor, the uncertainty of destinations is reduced. 
        We use half-hour time windows to split one day into 48 time slots.
        \item \textbf{Vehicle Type:} 
        It has three values: cars, buses, and trucks. 
        Intuitively, the trucks most probably go to areas with high cargo demand (e.g., industry parks) and buses often go to areas with a dense population (e.g., commercial districts or transportation hubs). Figure~\ref{fig:v_type_dest} shows the proportion of different vehicle types in different types of areas. We found only a few trucks go to the commercial areas; 
        cars and buses contribute major volume in the commercial and transportation hub areas, respectively.
    \end{itemize}

    \begin{figure}[htbp] \centering
    \vspace*{-5pt}
    \begin{minipage}{0.5\linewidth} \centering
        \vspace*{-5pt}
%         \hspace*{-30pt}
        \includegraphics[width=\linewidth, keepaspectratio=true]{fig/vehicle_type_area.pdf}
        \vspace*{-15pt}
        \caption{Dest. variance}
        \label{fig:v_type_dest}
        % \hspace*{5pt}
    \end{minipage}
    \hspace*{-5pt}
    \begin{minipage}{0.5\linewidth} \centering
        \vspace*{-5pt}
%         \hspace*{-30pt}
        \includegraphics[width=\linewidth, keepaspectratio=true]{fig/possible_destination.pdf}
        \vspace*{-15pt}
        \caption{Crowd dest.}
        \label{fig:crowd_dest}
    \end{minipage}
    \vspace*{-10pt}
    \end{figure}
    
    \textbf{Crowd Features:} The individual vehicle's historical data can be very sparse (as we suggested in Section~\ref{sec:moti}). we try to use the crowd destinations to provide complementary information. 
    Figure~\ref{fig:crowd_dest} shows the possible destinations from the same origins by different percentages of the total transactions (i.e., different crowd sizes). 
    For example, based on the $30\%$ of transaction data from the same origin (i.e., the 30\% curve), 
    almost $90\%$ of vehicles go to at most 4 destinations. It indicates lots of vehicles from the same origins share the similar destinations, which can be used to infer the destination of a vehicle without any historical destination data. 
    
    \textbf{Context Features:} We further consider other context features, i.e., day of week, weekday/weekend, holidays, that may have impacts on the destination choices. 
    We choose the 10 most popular destinations for each origin and compare the rank of these destinations in a regular day with that in other days with different contexts using the measurement of Normalized Discounted Cumulative Gain $NDCG$~\cite{jarvelin2002cumulated}. 
    The lower the $NDCG$, the lower similarity the destination choices. 
    Figure~\ref{fig:NDCG} shows that the measurement between weekdays, weekend, and holiday. 
    The holiday has very different destination choices compared to other days. 
    In the early morning and the late afternoon of weekends, the $NDCG$ is also lower than that of weekdays. It suggests these factors have impacts on people's choice of the destinations.
    
    \begin{figure}[htbp] \centering
    \vspace*{-2pt}
    \begin{minipage}{0.43\textwidth} \centering
        \vspace*{-5pt}
        \includegraphics[width=\textwidth, keepaspectratio=true]{fig/ndcg.pdf}
        \vspace*{-20pt}
    \end{minipage}
    \caption{Context impacts}
    \label{fig:NDCG}
    \vspace*{-15pt}
    \end{figure}

% To avoid this issue, we modify the order-$k$ Markov predictor to collaborate with the historical data of other vehicles.

% The order-$k$ Markov predictor can be briefly described as estimating the next location from a current context, which comprises the $k$ most recent locations. 
% Considering a vehicle whose location history is $L=a_1a_2\ldots a_n$. Given the current location context $c=k_{t-k+1}\ldots l_{t-1}l_t$ and the vehicle location as a random variable $X$, the transition probability of the vehicle $V_i$ to a future location $a$ is expressed as:

% \begin{equation}
% \begin{split}
%     P_{V_i}(X_{t+1}=a|L)
%     &=P(X_{i+k+1}=a|X(i+1, i+k)=c)\\
%     &=\frac{N(ca,L)}{N(c,L)},
% \end{split}
% \end{equation}
% where $N(c, L)$ denotes the number of times the substring $s$ occurs in the context $L$.

% To collaborate with other vehicles, we first define the similarity measurement between two vehicles.
% % Given the historical data $L_1$ and $L_2$ of two vehicles, we align their historical data and remain the data starting from the earliest same location. For example, if $L_1=a_1a_2a_3\ldots a_n$ and $L_2=a_2,a_4,\ldots a_m$, then the remaining 
% Given the historical data $L_1$ and $L_2$ of two vehicles $V_1$ and $V_2$, we use the Edit Distance~\cite{navarro2001guided} to represent the similarity $Sim(V_1,V_2)=Edit(L_1, L_2)$. Then the transition probability is adjusted as 
% \begin{equation}\label{eq:markov_adjust}
% \begin{split}
%     &P_{V_i}(X_{t+1}=a|L) \\
%     &= \frac{\sum_j Sim(V_i, V_j)P_{V_j}(X_{i+k+1}=a|X(i+1,i+k)=c)}{norm},
% \end{split}
% \end{equation}
% where $norm$ is the sum of $P_{V_i}$ on all the possible $a$. In equation~\ref{eq:markov_adjust}, the similarity between vehicles are used as weights to adjust the transition probability.
% Given estimates of all the future locations, we sample according to their probability to infer their next location.

\subsection{Route Predictor}
\label{sec:route_prediction}

Different from~\cite{xue2009traffic}, since the ETC transactions do not show which routes are used between particular origins and destinations, we first need to infer all historical routes of vehicles given a set of historical origin/destination pairs. In this paper, we focus on location prediction, and utilize the algorithm proposed in~\cite{yang2018sharededge} to obtain a historical route based on a pair of origin and destination along with the travel duration. 
Similar to the destination prediction, we study the features from three perspectives: individual features, crowd features and context features.



%Then identify a few features for route predictions.

% \subsubsection{\textbf{Historical Routes:}}
% Intuitively, the route choice are highly related to the highway network structure.
% The more complex the highway structure, the more possible routes.
% Theoretically, if we consider road structure as a pure graph, 
% there are infinite routes between a pair of origins and destinations 
% since one edge in the graph can be visited repetitively.
% It would be computationally expensive if we take all possible routes into consideration.
% To reduce the route candidates space, we have two observations: 
% (i) for a single trip, all people at most visit one edge once~\cite{}, and 
% (ii) people only use the shortest route or the routes that are reasonably longer than the shortest for short travel time (e.g., $50\%$ longer than the shortest path)~\cite{}.
% Given these two assumptions, we prune the entire route candidate space to a small size.
% among sampled local drivers by presenting these route candidates to them. 
% These drivers select all the possible paths in reality, which consist of our final route candidate space. We omit the survey results given space limitation. 

% In this work, we utilize a survey dataset from Guangdong ETC management company with the routes 14 thousand drivers will choose given a particular set of origins and destinations and a time of day, which were conducted for new highway planning. 
% With this route dataset, for each highway origin and destination pairs, we have a set of routes with selected counts, which are used as an offline route choice distribution. 

\textbf{Individual Features:} We utilize the following features for the route prediction at the individual level. 
    \begin{itemize}
        \item \textbf{Historical Routes:} 
        Based on a previous study, people are more reluctant to change their regular routes if they had more experience with these routes~\cite{ben2010road}, which indicates historical routes are most likely to be their future routes given the same trip or partially overlapped trips. 
        \item \textbf{Driving Experience:} Empirically, experienced people are good at finding the best routes among all the choices~\cite{ben2010road}. 
        We quantify the experience by two factors: 
        (i) the frequency of driving on highways, which can be obtained from historical ETC transactions; (ii) the saved travel time compared with the average travel time, which can also be computed from historical ETC data.
        \item \textbf{Time Factor:} Empirically, people generally have their own estimations about the route traffic at different time, e.g., taking a detour during the rush hour to avoid the traffic. It affects their future route choices.
    \end{itemize}
    
    \textbf{Crowd Features:}
    For those people who have no or only limited historical data, we incorporate the route choices of crowds to infer their route choice. Specifically, we use the probability of historical crowds' routes between particular origin/destination at the certain time.

    \textbf{Context Features:} 
    People's route choices are affected by the real-time context~\cite{ben2013impact}, i.e., day of week and real-time traffic speed. The detailed process of real-time traffic speed estimation is presented in next subsection.

% Considering the route choices of people are relatively stable~\ref{}, we study their historical route choices behaviors to infer the real-time chose route.
% The fundamental idea to infer the paths is that the total travel duration is the sum of the travel duration on each edges.
% Using the same approach in Section~\ref{sec:micro}, we can infer the driving speed of each vehicle in each edge. 
% With their driving speed and possible candidate paths, we can estimate their travel duration on each paths. 
% Then we select the one with minimum estimate error as the inferred path. The detailed process is given in Algorithm~\ref{alg:path}.

% \begin{algorithm}
% \caption{Historical Travel Path Inference}\label{alg:path}
% \SetKwInOut{Input}{Input}
% \SetKwInOut{Output}{Output}
% \underline{HTPI}{($h\_trans, c\_paths, D$)}\\
% \Input{historical transactions $h\_trans$,\\
%         candidate paths $c_paths$,\\
%         the total travel duration $D$}
% \Output{the inferred path}

% Estimate the historical crowd traffic speed $c\_speed$\\
% \tcc{apply the approach in \ref{sec:crowd_speed}}
% Estimate the individual traffic speed $i\_speed$\\
% \tcc{apply the approach in \ref{sec:indi_speed}}

% \For{$p$ in $c\_paths$}{
%     search the individual travel speed of edges on the path $p$\\
%     sum the travel duration on each edge of $p$\\
%     store the sum as $D_p$
% }
% return $\argmin\limits_{p}|D_p - D|$ 
% \end{algorithm}


% Given the estimated crowd traffic speed and its strong correlation with individual driving speeds, the intuitive approach is to use the regression model to estimate their speeds. 
% We apply the linear regression model to fit the individual driving speed and the average crowd traffic speed.
% The fitting and testing samples are split as $2/3$ and $1/3$ of the total size.
% Figure~\ref{fig:speed_err} shows CDF of the root mean square error in . 
% We can see there are more $40\%$ of the estimation with the errors over 5 $m/s$. 
% This error might be acceptable in some contexts.
% However, in our context of tracking, it may lead to hundreds meter location offsets compared to the real locations.

% \begin{figure}[htbp] \centering
%     \begin{minipage}{0.46\textwidth} \centering
%         \vspace*{-10pt}
% %         \hspace*{-30pt}
%         \includegraphics[width=\textwidth, keepaspectratio=true]{fig/speed_err_cdf.pdf}
%         \vspace*{-15pt}
%         % \hspace*{5pt}
%     \end{minipage}
%     \caption{Speed regression error}
%     \label{fig:speed_err}
%     \vspace*{-5pt}
% \end{figure}

\subsection{Speed Predictor}
\label{sec:speed_prediction}
In this subsection, we first introduce our features for speed prediction, and then we introduce in detail how we obtain generic crowd speeds as a crowd feature. 

\subsubsection{\textbf{Features:}} 
\label{sec:indi_speed}
We introduce our features on the individual, crowd, and context level.

     \textbf{Individual Features:} Since the driving speed is essentially based on people's behaviors, we define a set of individual vehicle's features.
    \begin{itemize}
        \item \textbf{Historical Driving Speed:} As shown in Figure~\ref{fig:speed_std}, the driving speed is relatively stable for a particular person. 
        We use their average speeds of historical trips to reflect their general driving speed.
        
        \item \textbf{Vehicle Type:} This feature reflects the vehicle's type (i.e., cars, buses, trucks). Intuitively, the driving speed of cars should be higher than trucks and buses. Figure~\ref{fig:v_type_speed} also validates this intuition.
        
        \item \textbf{Time Factor:} Figure~\ref{fig:v_type_speed} shows that the driving speed is different at different time of a day, which is mainly due to the different traffic condition.
    \end{itemize}

    \begin{figure}[htbp] \centering
        \vspace*{-5pt}
        \begin{minipage}{0.5\linewidth} \centering
            \vspace*{-5pt}
    %         \hspace*{-30pt}
            \includegraphics[width=\linewidth, keepaspectratio=true]{fig/vehicle_type_speed.pdf}
            \vspace*{-20pt}
            \caption{Speed variance}
            \label{fig:v_type_speed}
            % \hspace*{5pt}
        \end{minipage}
        \hspace*{-5pt}
        \begin{minipage}{0.5\linewidth} \centering
            \vspace*{-5pt}
    %         \hspace*{-30pt}
            \includegraphics[width=\linewidth, keepaspectratio=true]{fig/weather_speed.pdf}
            \vspace*{-20pt}
            \caption{Context impacts}
            \label{fig:context_speed}
        \end{minipage}
        \vspace*{-5pt}
    \end{figure}
    
    \textbf{Crowd Features:} People may behave differently under different traffic conditions. Instead of studying the detailed behavior patterns of individuals, which may have many factors to discuss, we directly investigate the correlation between the individual speed and crowd speed. Figure~\ref{fig:speed_cor} shows the Pearson correlation of the individual speed and crowd traffic speed. More than 80$\%$ of vehicles have at least 0.89 correlation coefficient with the crowd traffic speed. Motivated by the strong correlation, the crowd traffic speed is an important feature to estimate the individual driving speeds on specific edges.
    Therefore, we extract the features of the vehicle speed samples, which are incorporated to estimate the crowd traffic speed. Instead of using the average crowd traffic speed (which may cause estimation bias), we consider the statistic values of the crowd traffic speed distribution estimated in the next subsection~\ref{sec:crowd_speed}. Especially, we use letter values of the distribution, including minimum, lower fourth, median, upper fourth and maximum of the samples.
    
    \begin{figure}[htbp] \centering
    \begin{minipage}{0.43\textwidth} \centering
        \vspace*{-10pt}
        \includegraphics[width=\textwidth, keepaspectratio=true]{fig/traffic_speed_cor.pdf}
        \vspace*{-20pt}
    \end{minipage}
    \caption{Speed Correlation}
    \label{fig:speed_cor}
    \vspace*{-5pt}
    \end{figure}
    
    % \begin{figure}[htbp] \centering
    %     \vspace*{-5pt}
    %     \begin{minipage}{0.5\linewidth} \centering
    %         \vspace*{-5pt}
    % %         \hspace*{-30pt}
    %         \includegraphics[width=\linewidth, keepaspectratio=true]{fig/traffic_speed_cor.pdf}
    %         \vspace*{-18pt}
    %         \caption{Speed Correlation}
    %         \label{fig:speed_cor}
    %         % \hspace*{5pt}
    %     \end{minipage}
    %     \hspace*{-5pt}
    %     \begin{minipage}{0.5\linewidth} \centering
    %         \vspace*{-5pt}
    % %         \hspace*{-30pt}
    %         \includegraphics[width=\linewidth, keepaspectratio=true]{fig/weather_speed.pdf}
    %         \vspace*{-20pt}
    %         \caption{Context impacts}
    %         \label{fig:context_speed}
    %     \end{minipage}
    %     \vspace*{-5pt}
    % \end{figure}
        
    \textbf{Context Features:} Besides the vehicle-related features, we also consider other factors that may have impacts on the driving speed, including weather and weekday/weekend. As shown in Figure~\ref{fig:context_speed}, the speed is decreased by $10\%$ at most in the rainy day and increased by $5\%$ on weekend. This is reasonable because people tend to drive slower when raining and less people use highways to work on the weekend, which makes the highways less congested.

\subsubsection{\textbf{Crowd Traffic Speed Estimation}}
\label{sec:crowd_speed}
Without any GPS locations of vehicles, a straightforward method is to use the duration of one-edge trips to directly obtain the travel speed on that edge, which is based on whether we have enough one-edge trips to cover all the edges. 
Figure~\ref{fig:route_length} depicts the trip length in term of edges. 
It shows there are only $18\%$ of the trips from the same day are one-edge trips.
We map these edges covered by one-edge trips onto the highway structure and find only $22\%$ of all edges on the highway are covered (shown in Figure~\ref{fig:edge_coverage}). 
But if we include some slight-longer trips, e.g., two-edge trips and three-edge trips, we can cover a majority of edges with $82\%$ in the peak hours through computing the difference between shorter and longer trips. 
The coverage in the early morning is still lower. However, since the traffic is light during the early morning, the traffic speed can be approximated as free-flow speed~\cite{wang2014impact}.

\begin{figure}[htbp] \centering
    \begin{minipage}{0.5\linewidth} \centering
        \vspace*{-5pt}
%         \hspace*{-30pt}
        \includegraphics[width=\linewidth, keepaspectratio=true]{fig/route_length_edge.pdf}
        \vspace*{-15pt}
        \caption{Trip length}
        \label{fig:route_length}
        % \hspace*{5pt}
    \end{minipage}
    \hspace*{-5pt}
    \begin{minipage}{0.5\linewidth} \centering
        \vspace*{-5pt}
%         \hspace*{-30pt}
        \includegraphics[width=\linewidth, keepaspectratio=true]{fig/edge_coverage.pdf}
        \vspace*{-15pt}
        \caption{Edge coverage}
        \label{fig:edge_coverage}
    \end{minipage}
    \vspace*{-5pt}
\end{figure}

As a result, we collaboratively estimate the traffic speeds with other trips with more edges.
The basic idea is illustrated as an example in Figure~\ref{fig:demo}.
Given three trips Trip$_A$, Trip$_B$, Trip$_C$ with travel duration $d_A, d_B, d_C$, 
their routes are $e_1$, $e_1e_2$ and $e_1e_2e_3$, respectively, since shorter trips are less uncertain. 
By comparing the travel duration of Trip$_A$ and Trip$_B$, we can estimate the travel duration on $e_2$ as $d_B-d_A$, which can be transformed into the traffic speed on $e_2$ given the travel distance.
Similarly, the traffic speed of $e_3$ can be estimated by Trip$_B$ and Trip$_C$.
Note that there can be multiple Trip$_B$ and Trip$_C$ from different vehicles to estimate the traffic speed on $e_3$, which make it more robust to outliers.

\begin{figure}[htbp] \centering
    \begin{minipage}{0.40\textwidth} \centering
        \vspace*{-10pt}
%         \hspace*{-30pt}
        \includegraphics[width=\textwidth, keepaspectratio=true]{fig/speed_estimation.pdf}
        \vspace*{-15pt}
        % \hspace*{5pt}
    \end{minipage}
    \caption{Demo of crowd traffic speed estimation}
    \label{fig:demo}
    \vspace*{-10pt}
\end{figure}


% One prerequisite of using short trips with less uncertainty route is that the trips should cover as much as the edges on highways.

% Incorporating trips with more edges may potentially increase the coverage but also brings issues such as uncertain routes and computation complexity.
% %and uncertainty (i.e., the speed variance can be greater in longer routes).
% To prevent these issues, we simplify the estimation for the rest $x\%$ uncovered edges using that of the adjacent edges.



% The detailed algorithm of the crowd traffic speed estimation is shown in Algorithm~\ref{alg:macro}.

% \begin{algorithm}
% \caption{Crowd Traffic Speed Estimation}\label{alg:macro}
% \SetKwInOut{Input}{Input}
% \SetKwInOut{Output}{Output}
% \underline{CTSE}{($k-edge,all_edges$)}\\
% \Input{k-edge trips(k=1,2,3) $k-edge$, all the edges $edges$}
% \Output{Crowd traffic speed on each edge}

% Label the edge travel time using $1-edge$;\\
% \For{$k$ in $2,3$}{
%     \For{$transaction$ in $k-edge$}{
%         $e_{labeled}, e_{unlabeled}, duration$ = $transaction$\\
%         label $e_{unlabeled}$ as $\frac{duration-duration_{e_{unlabeled}}}{length(e_{unlabeled})}$
%     }
% }
% \For{$e$ in all $e_{unlabeled}$}{
% label $e$ as the traffic speed of the adjacent edge
% }
% return all traffic speed of $all_edges$
% \end{algorithm}

However, a key issue of the method is that the travel duration difference used to obtain the edge travel time is from different vehicles, which lead to errors due to different driving behaviors.  
For example, in Figure~\ref{fig:demo}, the derived duration on $e_2$ is the subtraction of $d_A$ and $d_B$ which are from two different vehicles. 
Even though we could have multiple derived durations on $e_2$, since each of them is obtained from two different users, their variance is high. 
To providing robust estimation, we form the problem as a parameter estimation problem. 
Given multiply derived duration as samples, our goal is to find the true distribution (i.e., true speed distribution in each edge).
Instead of using the average of multiply derived duration on an edge $e_n$, we consider the traffic speed of $e_n$ as a distribution with mean $\mu_n$ and variance $\sigma^2$.


% For better illustration, we name the duration from the actual trips (e.g., $d_A, d_B, d_C$) as actual duration samples and estimated duration (e.g., duration on $e_2$ by $d_B-d_A$) as derived duration samples in the following sections.



%If the actual driving duration on $e_1$ of trip A is largely different from $d_A$, then it may increase the error of the duration estimation on $e_2$.

A key problem in the parameter estimation is to measure the confidence of the used samples, which are a set of derived durations in our setting.  
The confidence is described as the difference between derived duration samples and the actual travel duration (i.e., obtained directly from single-edge trips).
% The confidence of derived duration samples can vary depending on how similar the actual duration samples are to obtain the derived duration samples.
Intuitively, the more similar the driving habits of two persons (i.e., average driving speed), the more confident the derived duration samples.
Motivated by this intuition, we modify the formula in~\cite{wang2017discovering} and define the confidence as follows:
\begin{equation}
    u_{ij}^{e_n} = 1 - exp(-s^2/\lambda)
\end{equation}
where $s=(l_n/d_i) - (l_n/d_j)$, $l_n$ is the length of the edge $e_n$, $d_i$ and $d_j$ are the two actual durations used to derive the duration on $e_n$, $\lambda$ is the parameter to control the trend of $u_{ij}^{e_n}$.

Given the definition of the confidence, combining all the one-edge, two-edge and three-edge, we have speed samples with confidence coefficients on different edges. 
Those coefficients are regarded as the weight of the sample. 
Then our objective is to estimate the true speed distribution of each edge, which most probably generates the weighted samples.
The objective function can be formulated as follows:
\begin{equation}
    \theta^t = \argmax\limits_{\theta^t}\sum\limits_{e}\log p(S_{e}|\theta^t)
\end{equation}
where $\theta^t$ is the distribution parameter at time $t$, $e$ is the edge, $S_e^t$ is the sample collection on edge $e$ at time $t$.

According to~\cite{lo2013expectation}, we assume the traffic speed distribution as a Gaussian Mixed Model(GMM). 
To solve the objective function, we adopt Expectation Maximization algorithm~\cite{bilmes1998gentle} to estimate the parameters. 
Due to the space limitation, we omit the detailed derivation steps, which can be found in~\cite{bilmes1998gentle}.

The travel duration given by ETC data include driving time on ramps when a vehicle enters or leaves the highway. Based on different geographic features of highway toll stations, some ramps may be long and people usually slow down after they enter ramps, which leads to our travel speed calculation for highway edges associated with them less accurate. 
In this work, we estimate the travel time on ramps based on the ramp length compared to the highway edge length to improve our travel speed estimation.

% Besides the sample data, we also introduce spatial-temporal constrains on the traffic speed distribution. For example, the adjacent edges have similar traffic pattern in general and traffic speed between adjacent time slots also maintains continuity~\cite{deng2016latent}.
% Given these two constrains, we modify the objective function as follows:
% \begin{equation}
%     \theta^t = \argmax\limits_{\theta^t}\sum\limits_{e}\log p(S_{e};\theta^t)
% \end{equation}


\subsection{Learning with Mondrian Forest}
Mondrian forests~\cite{lakshminarayanan2014mondrian} is an online random forest model using Mondrian processes to construct ensembles of random decision trees. 
Compared to the offline or online random forest~\cite{lakshminarayanan2014mondrian}, it provides the ability to process online data and online updates faster and more accurately.
Compared with other algorithms, the Mondrian forests model has the following advantages:
\begin{itemize}
    \item It is more robust to heterogeneous features. In our data input, we have both numerical variables (i.e., speed) and categorical values (i.e., vehicle type, weather, weekday/weekend). These variables can be input into the model directly without conversion or normalization.
    \item It provides self-check on the importance of the features during the training stage. For example, such as the weather condition and holidays, these variables would only have high importance under certain conditions with a low frequency.
    %\item It is efficient for large data input. Considering the huge volume in ETC systems, it ensures the real-time effects of the estimation.
    \item Compared to other neural based model (e.g., deep neural network), the results are more interpretable because of the internally used decision tree~\cite{friedman2001elements}.
\end{itemize}

For different tasks (i.e., destination prediction, route inference, speed estimation), we fit all the extracted features into Mondrian forests and learn three predictors to work collaboratively the real-time location prediction, which is illustrated in Section~\ref{sec:together}.

\subsection{Put them all together}
\label{sec:together}
In the previous sections, we have conducted analysis on the three key tasks: destination prediction, route inference and speed estimation.
Based on multiple extracted features, we learn three predictors \textit{d-predictor, r-predictor, s-predictor} for each of the tasks, perceptively. The procedure of real-time location prediction is described in Algorithm~\ref{alg:algo}.

\begin{algorithm}
\caption{Real-time Location Prediction}\label{alg:algo}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{\textit{d-predictor}: the destination predictor,\\
        \textit{r-predictor}: the route predictor,\\
        \textit{s-predictor}: the speed predictor,\\
        $entrance$: the entering toll station,\\
        $t_0$: the entering time.}
\Output{real-time locations}
$destination\leftarrow$ \textit{d-predictor} given $entrance$\\
$route\leftarrow$ \textit{r-predictor} given $destination$\\
$distance$ = 0\\
\While{$distance$ < $route.length$}{
    $speed\leftarrow$ \textit{s-predictor} at $t_i$\\
    $distance$ += $speed\times interval$\\
    $location\leftarrow$ match $distance$ to $route$\\
}
\end{algorithm}

% In VeMo system, there are three kinds of feedbacks that can be directly observed in real time, including

% \noindent \textbf{Wrong Destination}: A vehicle leaves the highways from a toll station other than the predicted exit before or after the expected arrival, i.e., \textit{d-predictor} is wrong.

% \noindent \textbf{Early Arrival}: A vehicle leaves the highways earlier than predicted. It could be a wrong prediction in either the route, the speed, or both.

% \noindent \textbf{Late Arrival}: A vehicle arrives at the exit station later than expected. Similarly, it could be a wrong prediction in either the route, the speed, or both.
% \begin{itemize}
%     \item \textbf{Wrong Destination}: A vehicle leaves the highways from a toll station other than the predicted exit before or after the expected arrival, i.e., \textit{d-predictor} is wrong.
    
%     \item \textbf{Early Arrival}: A vehicle leaves the highways earlier than predicted. It could be a wrong prediction in either the route, the speed, or both.  
    
%     \item \textbf{Late Arrival}: A vehicle arrives at the exit station later than expected. Similarly, it could be a wrong prediction in either the route, the speed, or both. 
% \end{itemize}

% Instead of remaining the system unchangeable, we make use of these three kinds of feedback to provide online updating ability for the system for self-awareness. 
% In particular, we utilize wrong destinations for a particular vehicle to update its historical destination; we utilize early or late arrival to further update real-time speed predictions and routes by adjusting input features for s-predictor and r-predictor. Due to the space limitation, we omit the updating process, which follows the online updating described in~\cite{lakshminarayanan2014mondrian}.
